Molecular hydrogen abundances of galaxies in the EAGLE simulations

We investigate the abundance of galactic molecular hydrogen (H$_2$) in the "Evolution and Assembly of GaLaxies and their Environments" (EAGLE) cosmological hydrodynamic simulations. We assign H$_2$ masses to gas particles in the simulations in post-processing using two different prescriptions that depend on the local dust-to-gas ratio and the interstellar radiation field. Both result in H$_2$ galaxy mass functions that agree well with observations in the local and high-redshift Universe. The simulations reproduce the observed scaling relations between the mass of H$_2$ and the stellar mass, star formation rate and stellar surface density. Towards high edshifts, galaxies in the simulations display larger H$_2$ mass fractions, and correspondingly lower H$_2$ depletion timescales, also in good agreement with observations. The comoving mass density of H$_2$ in units of the critical density, $\Omega_{\rm H_2}$, peaks at $z\approx 1.2-1.5$, later than the predicted peak of the cosmic star formation rate activity, at $z\approx 2$. This difference stems from the decrease in gas metallicity and increase in interstellar radiation field with redshift, both of which hamper H$_2$ formation. We find that the cosmic H$_2$ budget is dominated by galaxies with $M_{\rm H_2}>10^9\,\rm M_{\odot}$, star formation rates $>10\,\rm M_{\odot}\,\rm yr^{-1}$ and stellar masses $M_{\rm stellar}>10^{10}\,\rm M_{\odot}$, which are readily observable in the optical and near-IR. The match between the H$_2$ properties of galaxies that emerge in the simulations and observations is remarkable, particularly since H$_2$ observations were not used to adjust parameters in EAGLE.

==> app_apertures.tex <==
\section[]{The effect of aperture measurements in the H$_2$ mass function}\label{Apertures}

In Fig.~\ref{AperH2MF} we show the H$_2$ mass function for the 
simulation Ref-L100N1504 when the H$_2$ mass is measured in individual sub-halos in apertures 
of $30$pkpc, $60$pkpc and when all the H$_2$ mass within the sub-halo is included.

%\begin{figure}
%\begin{center}
%\includegraphics[trim = 1.5mm 0.5mm 1mm 1mm,clip,width=0.49\textwidth]{Figs/PDFsFromPadilla14Mergers.eps}
%\caption{As in Fig.~\ref{PDFs} but here we show the flips in the angular momentum of DM halos only due to mergers 
%with other DM halos. The fractional change in mass due to mergers are as labelled in the top panel.}
%\label{AperH2MF}
%\end{center}
%\end{figure}



==> app_boxcomparison.tex <==
\section[]{Analysis of simulation volumes}\label{BoxComparison}

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{Figs/EAGLE_H2MassFunction_HighRedshifts_BothModels_TestBoxEffects.eps}
\caption{The H$_2$ mass functions for the reference simulation Ref-L100N1504 (solid lines) and Ref-L050N0752 (dashed lines) 
using the GK11 prescription and at three different redshifts, as labelled. Observations are as in Fig.~\ref{H2MFHighz}.}
\label{H2MFBoxComp}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[width=0.45\textwidth]{Figs/EAGLE_OmegaH2_v2_TestBoxSize.eps}
\caption{$\Omega_{\rm H_2}$ as a function of redshift for the simulations Ref-L100N1504 (solid lines) and Ref-L050N0752 (dashed lines) 
with the GK11 prescription applied.
 Observations are as in Fig.~\ref{OmegaH2}.}
\label{OmegaH2BoxComp}
\end{center}
\end{figure}


Here we compare the simulations Ref-L100N1504 and Ref-L050N0752 to address the effect of the simulated volume.
Fig.~\ref{H2MFBoxComp} shows the H$_2$ mass functions at $z=0$ (top panel), $z=1.2$ (middle panel) and $z=2.3$ (bottom panel) for the simulations 
Ref-L100N1504 (solid lines) and Ref-L050N0752 (dashed lines) with the GK11 prescription applied. 
The number densities of the two simulations at $M_{\rm H_2}>10^{9.5}\,\rm M_{\odot}$ agree very well in the 
 range where they overlap. For example, at $z=1.2$ the number density of galaxies with $M_{\rm H_2}\gtrsim 10^{10}\,\rm M_{\odot}$  
in the simulation Ref-L050N0752 is $4$, while in the Ref-L100N1504 is $26$, which is consistent with the increase in volume 
by a factor of $8$. 

We show in Fig.~\ref{OmegaH2BoxComp} the evolution of $\Omega_{\rm H_2}$ for the simulations Ref-L100N1504 and Ref-L050N0752 
and find they agree within $15$\%, again showing that the contribution to the H$_2$ content of the universe from massive galaxies 
that are not well sampled in the simulations Ref-L100N1504 and Ref-L050N0752 is very unlikely.
We conclude that the comparison between Ref-L100N1504 and the observations presented in $\S$~\ref{RedEvoSec} 
is robust.


